Geometric phase and its applications: topological phases, quantum walks and non-inertial quantum systems

Geometric phase plays a fundamental role in quantum theory and accounts for wide phenomena ranging from the Aharanov-Bohm effect, the integer and fractional quantum hall effects, and topological phases of matter, including topological insulators, to name a few. In this thesis, we have proposed a fresh perspective of geodesics and null phase curves, which are key ingredients in understanding the geometric phase. We have also looked at a number of applications of geometric phases in topological phases, quantum walks, and non-inertial quantum systems. The shortest curve between any two points on a given surface is a (minimal) geodesic. They are also the curves along which a system does not acquire any geometric phase. In the same context, we can generalize geodesics to define a larger class of curves, known as null phase curves (NPCs), along which also the acquired geometric phase is zero; however, they need not be the shortest curves between the two points. We have proposed a geometrical decomposition of geodesics and null phase curves on the Bloch sphere, which is crucial in improving our understanding of the geometry of the state space and the intrinsic symmetries of geodesics and NPCs. We have also investigated the persistence of topological phases in quantum walks in the presence of an external (lossy) environment. We show that the topological order in one and two-dimensional quantum walks persist against moderate losses. Further, we use the geometric phase to detect the non-inertial modifications to the field correlators perceived by a circularly rotating two-level atom placed inside a cavity.

==> others/acknowledgments.tex <==
\begin{center}
{\Large \em \textbf{Acknowledgments}}
\end{center}
\textbf{sigh} and \textbf{yayyyyyyyy!!!}

This roller coaster ride has come to an end. It has been a long journey and a truly unique life experience. My path crossed with many people who made this journey fulfilling and meaningful, and this work would not exist (like any other work) without the support and guidance of these people. 

First, I would like to express my deepest gratitude to my supervisor and mentor, Dr. Sandeep K. Goyal, for giving me the opportunity to work with him, providing continuous encouragement, and being available for discussions virtually all the time. His expertise in several fields and his enthusiasm to work in diverse areas were invaluable in formulating the research problems. I want to also thank him and his wife Anshu for hosting us infinite times for dinner with delicious food and drinks at their home.

I am grateful to my doctoral committee members, Dr. Sanjeev Kumar, Prof. Kavita Dorai, and Dr. Manabendra Nath Bera, for their time, support, and constant guidance. I would also like to thank my collaborators, Dr. Sanjib Dey, Dr. Kinjalk Lochan, Dr. Akhilesh K.S., and Navdeep Arya, for sharing their expertise, which further helped me to broaden my horizon. Discussions with Navdeep over long walks were of great help in understanding the subtlety and beauty of physics. His constructive criticism always encouraged me to go one step ahead and helped me ask the right questions.

I am blessed to have excellent teachers who gave me the appropriate tools and guidance to choose the right path. A special mention to Dr. Indira Santhanam and Dr. Namrata Diwan Soni from Hansraj College, Prof. Arvind, Dr. Abhishek Choudhuri, and Dr. Mandip Singh from IISER Mohali.

I would also like to thank IISER Mohali, Ministry of Human Resource and Development (MHRD) and Interdisciplinary Cyber Physical Systems (ICPS) programme of the Department of Science and Technology, India (Grant No. DST/ICPS/QuST/Theme-1/2019/12)
for providing me with financial assistance during my Ph.D. tenure. 

I am very thankful to all the non-teaching staff, the Offices of the Dean Students, Dean Academics, and Dean R\&D, accounts section, library and its staff for their assistance. I would also like to mention hostel caretakers, mess people, cleaning staff, Lala Ji and his family and Bisu bhaiya from the canteen, and the entire IISER Mohali community for their help and cooperation during my stay at IISER Mohali. 

Without mentioning my huge, extended, family at IISER Mohali, this acknowledgment will not be complete. This includes \emph{Miles}, the IISER Mohali running club, and our Yog Parivar. It is impossible to list them all because I will definitely miss someone out, which would be an injustice. I want to express my deepest gratitude to all of them from the bottom of my heart for making my life at IISER Mohali incredibly joyful and an unforgettable journey. With a special mention to the people who helped me to their total capacity when I got infected with the Coronavirus. I would also like to acknowledge the 2014 B.Sc(Honors) Physics batch, especially the \emph{Chupeshtanuse} group from Hansraj college, for introducing me to the real world. 

Finally, I owe my deepest gratitude and love to my parents and brothers for their constant support. Without my family, I would not be who I am right now. Even though my parents were not educated enough, they always supported my studies and encouraged me to pursue my dream of contributing to science one day.


\begin{flushright}
	Vikash Mittal
\end{flushright}

==> others/certificate.tex <==
\begin{center}
{\Large Certificate of Examination}
\end{center}
\vspace{1.0cm}
This is to certify that the dissertation titled \emph{“\thesistitle”} submitted by {\bf \candidate} (Reg. No. \registration) for the partial fulfillment of \degree~programme of the Institute, has been examined by the thesis committee duly appointed by the Institute. The committee finds the work done by the candidate satisfactory and recommends that the report be accepted.
\vspace{1.5cm}

\begin{minipage}[t]{0.3\textwidth}
	\begin{center} 
		Prof. Kavita Dorai
	\end{center}
\end{minipage}
%
\begin{minipage}[t]{0.3\textwidth}
	\begin{center} 
		Prof. Sanjeev Kumar
	\end{center}
\end{minipage}
%
\begin{minipage}[t]{0.3\textwidth}
	\begin{center} 
		\supervisor \\
		(Supervisor)
	\end{center}
\end{minipage}


==> others/declaration.tex <==
\begin{center}
{ \Large \textbf{Declaration}} 
\end{center}
\vspace{1.0cm}
The work presented in this thesis has been carried out by me under the guidance of \supervisor~ at the Indian Institute of Science Education and Research Mohali. This work has not been submitted in part or in full for a degree, a diploma, or a fellowship to any other university or institute. Whenever contributions of others are involved, every effort is made to indicate this clearly, with due acknowledgment of collaborative research and discussions. This thesis is a bona fide record of original work done by me and all sources listed within have been detailed in the bibliography.

\begin{flushright}
\textbf{\candidate }\\
\vspace{0.5cm}
Place: \rule{3cm}{0.3mm} \\
Date: \rule{3cm}{0.3mm}

\end{flushright}
\vspace{1.0cm}
In my capacity as the supervisor of the candidate’s thesis work, I certify that the above statements by the candidate are true to the best of my knowledge.
\vspace{1.5cm}
\begin{flushright}
\textbf{\supervisor} \\
Assistant professor \\
Department of Physical Sciences \\
IISER Mohali \\
\vspace{0.5cm}
Place: \rule{3cm}{0.3mm} \\
Date: \rule{3cm}{0.3mm}
\end{flushright}


==> others/synopsis_title.tex <==
\begin{titlepage}
	
	\vfill
	\begin{center}
		\vfill
		\Large \textit{\textbf{Thesis Synopsis} }\\[0.1cm] % University requirement text
		\vfill
		
		\vfill
		{\huge {\thesistitle} \par}\vspace{0.01cm}
		\vfill
		
		{\Large \candidate \; (MP14011) \vskip 0.3cm Supervisor: \supervisor} 
		\vfill
		
		\centering
		\includegraphics[width=3.5cm]{logo}
		\vfill
		\department
		\\
		\vspace{0.5cm}
		\university
		\vfill
		{\date{January 2022}}
	\end{center}
	\vfill
	
\end{titlepage}



